On the Decentralized Generation of theRSA Moduli in Multi-Party Settings

RSA cryptography is still widely used. Some of its applications (e.g., distributed signature schemes, cryptosystems) do not allow the RSA modulus to be generated by a centralized trusted entity. Instead, the factorization must remain unknown to all the network participants. To this date, the existing algorithms are either computationally expensive, or limited to two-party settings. In this work, we design a decentralized multi-party computation algorithm able to generate efficiently the RSA modulus.

==> discussion.tex <==
\section{Discussion}\label{sec:security}
Here, we will share our thoughts about the security of the generalized protocol described in Section~\ref{sec:generalization}. We relax the honest node assumption, and we now allow the presence of malicious agents. We assume these nodes can send false informations to other nodes, but they have no physical access to other hardware and cannot intercept any communication. 

Under these assumptions, we claim that these malicious agents can only delay the key generation, and have negligible chances of retrieving the shared parts of the keys. In the following, we sketch the reasoning that brings us to this conjecture.

\subsubsection*{Fast trial division}
Compared to the Frederiksen protocol, we removed the $1$-out-of-$\beta$ OT which was resource-consuming and asking parties to communicates their secrets parts modulus small prime numbers. However, we don't think this represent a serious knowledge leak because it is possible to retrieve information only during the first round and as we change the communicating pairs each time it is really hard for an adversary to derive the original values even if they collude.

\subsubsection*{Distributed multiplication}
In this part the security should not be affected because we kept the same mechanism as the original protocol then leakage from communications is not possible.

However we have to consider the case in which the malicious agents try to send false values in order to generate non-biprime numbers. As we deal with random secret parts, this is not likely to change the probability of primeness of $p$ and $q$.

\subsubsection*{Biprimality test}
In these tests, we expect a value of $1$ each time. It is then impossible for a malicious party to guess values to fake in order to pass the tests each time. The greater $s$ is the more complicated it gets.

Finally, would an agent able to generate a non-biprimal number, it would be unable to guess the prime factors from random although it knows there are far less.
